Towards Enhancing Coherence in Extractive Summarization: Dataset and Experiments with LLMs

Extractive summarization plays a pivotal role in natural language processing due to its wide-range applications in summarizing diverse content efficiently, while also being faithful to the original content. Despite significant advancement achieved in extractive summarization by Large Language Models (LLMs), these summaries frequently exhibit incoherence. An important aspect of the coherent summary is its readability for intended users. Although there have been many datasets and benchmarks proposed for creating coherent extractive summaries, none of them currently incorporate user intent to improve coherence in extractive summarization. Motivated by this, we propose a systematically created human-annotated dataset consisting of coherent summaries for five publicly available datasets and natural language user feedback, offering valuable insights into how to improve coherence in extractive summaries. We utilize this dataset for aligning LLMs through supervised fine-tuning with natural language human feedback to enhance the coherence of their generated summaries. Preliminary experiments with Falcon-40B and Llama-2-13B show significant performance improvements (~10% Rouge-L) in terms of producing coherent summaries. We further utilize human feedback to benchmark results over instruction-tuned models such as FLAN-T5 which resulted in several interesting findings. Data and source code are available at https://github.com/Mihir3009/Extract-AI.

==> 02_related_work.tex <==
\section{Related Work}

\paragraph{Prior Datasets} \mihir{Write about existing datasets for extractive summarization and show how our dataset is different}

\paragraph{Prior Methods}
There are some past attempts that have been made to improve coherence in extractive summarization. \citet{christensen-etal-2013-towards} proposed a G-FLOW, a joint model for selection and ordering sentences that balances coherence for multi-document extractive summarization. After that, \citet{Parveen2015IntegratingIN} proposed a graph-based method for extractive single-document summarization that considers importance, non-redundancy, and local coherence simultaneously. Furthermore, \citet{Wu2018LearningTE} utilized reinforcement learning to extract a coherent summary, and \citet{Abdolahi2019TextualCI} enhanced coherence in extractive document summarization through a greedy approach and word vectors. In addition, \citet{Jie2023EnhancingCO} introduced two strategies, including pre-trained converting models (model-based) and converting matrices (MAT-based) that merge sentence representations to improve coherence. With the emergence of LLMs, \citet{zhang2023benchmarking} attempted to analyze the performance of GPT-3 with different prompting for generating coherent summaries. Differing from these existing efforts, we approach the concept of coherence within summaries through the lens of user-specific intent. \hanieh{I think this section needs expanding and organization. Maybe describe each work a bit more and categorize the previous methods a bit rather than listing them.}

% We conducted a literature search and found that improving coherence in extractive summarization is under-explored. However, there are some past attempts have been made in this research direction. Some of the interesting studies I have cited here as well. For example, Christensen et al., 2013 [6] propose a G-FLOW, a joint model for selection and ordering sentences that balances coherence for multi-document extractive summarization. After that, Parveen et al., 2015 [7] proposed a graph-based method for extractive single-document summarization that considers importance, non-redundancy, and local coherence simultaneously. Furthermore, Wu et al., 2018 [8] utilized reinforcement learning to extract a coherent summary, and Abdolahi et al., 2019 [9] enhanced coherence in extractive document summarization through a greedy approach and word vectors. In addition, Jie et al., 2023 [1]  introduced two strategies, including pre-trained converting models (model-based) and converting matrices (MAT-based) that merge sentence representations to improve coherence. With the emergence of LLMs, Zhang et al., 2023 [10] attempted to analyze the performance of GPT-3 with different prompting for generating coherent summaries.

% Differing from these existing efforts, we approach the concept of coherence within summaries through the lens of user-specific intent. In the following section, I will provide a more detailed description of the proposed method.

==> tables/enc_dec_results.tex <==
\begin{table}[h]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc}
\toprule
\textbf{Model}    & \textbf{Baseline} & \textbf{w/ Feedback} & \textbf{Pre-finetuning} \\ \midrule
FLAN-T5     & 67.74             & 46.78                   & \textbf{72.34}                            \\
Tk-Instruct & 65.62             & 45.44                   & \textbf{70.69}                            \\
T5          & 65.68             & 45.98                   & \textbf{71.78}                            \\ \bottomrule
\end{tabular}
}
\caption{Enc. + Dec. Models}
\label{tab:enc_dec_results}
\end{table}
